Multi-View Azimuth Stereo via Tangent Space Consistency

We present a method for 3D reconstruction only using calibrated multi-view surface azimuth maps. Our method, multi-view azimuth stereo, is effective for textureless or specular surfaces, which are difficult for conventional multi-view stereo methods. We introduce the concept of tangent space consistency: Multi-view azimuth observations of a surface point should be lifted to the same tangent space. Leveraging this consistency, we recover the shape by optimizing a neural implicit surface representation. Our method harnesses the robust azimuth estimation capabilities of photometric stereo methods or polarization imaging while bypassing potentially complex zenith angle estimation. Experiments using azimuth maps from various sources validate the accurate shape recovery with our method, even without zenith angles.

==> sections/figures_tables/fscore.tex <==
\begin{table}
	\definecolor{Gray}{gray}{0.85}
	\centering
	\caption{F-score ($\uparrow$)~\cite{kaya2022uncertainty,knapitsch2017tanks} of recovered geometry on DiLiGenT-MV benchmark~\cite{li2020multi}.}
	\resizebox{\linewidth}{!}{
		\begin{tabular}{@{}lrrrrrr@{}}
			\toprule
			& Bear & Buddha & Cow & Pot2 & Reading & Average \\
			\midrule
			%			Park16~\cite{park2016robust}  & 0.599 & 0.877 & 0.905 & 0.437 & 0.729 & 0.709  \\
			%			Li20~\cite{li2020multi} & 0.852 & 0.929 & 0.858 & 0.882 & 0.827 & 0.870\\
			%			Kaya22~\cite{kaya2022uncertainty} &  0.895 & 0.922 & 0.979 & 0.907 & \textbf{0.970} & 0.935\\
			%			Yang22~\cite{} &  &  &  &  &  & \\ 
			%%			\addlinespace
			%			Ours &\textbf{0.990}& \textbf{0.956} & \textbf{0.990} & \textbf{0.988} & 0.895 &  \textbf{0.962}\\
			%			Park16~\cite{park2016robust}  & 0.270 & 0.711 & 0.772 & 0.212 & 0.531 &   \\
			%			Li20~\cite{li2020multi} & 0.955 & 0.855 & 0.974 & 0.918 & 0.909 & \\
			%			Kaya22~\cite{kaya2022uncertainty} & 0.723  & 0.694 & 0.813 & 0.699 & 0.773  & \\
			%			Yang22~\cite{} &  0.896 & 0.807 & 0.857 & 0.914 & 0.772 & \\ 
			%			Ours & 0.900 & 0.768 & 0.898 & 0.959 & 0.566 &  \\
			Park16~\cite{park2016robust}  & 0.262 & 0.698 & 0.760 & 0.198 & 0.519 & 0.487  \\
			Li20~\cite{li2020multi} & \textbf{0.958} & \textbf{0.902} & \textbf{0.986} & 0.946 & \textbf{0.914} & \textbf{0.941}\\
			Kaya22~\cite{kaya2022uncertainty} & 0.707 & 0.669 & 0.798 & 0.731 & 0.762  & 0.733\\
			Yang22~\cite{} & 0.898  & 0.806 & 0.856 & 0.919 & 0.785 & 0.853\\ 
			Ours (SDPS) &0.909 & 0.754 & 0.907 & \textbf{0.962} & 0.546 & 0.816 \\
			\bottomrule
		\end{tabular}
	}
	\label{tab.fscore_mvps}
\end{table}

==> sections/figures_tables/pandora.tex <==
\begin{figure}
	\scriptsize
	\centering
	\newcommand{\figwidth}{0.2}
	\begin{tabular}{@{}cccc@{}}
		\begin{tabular}{c}
			color images \& \\
			polar-azimuth
		\end{tabular} & 
		Colmap~\cite{schoenberger2016mvs} & 
		PANDORA~\cite{dave2022pandora} &
		MAS (ours)
		\\
		    \begin{minipage}{\figwidth \linewidth}  \includegraphics[width= \linewidth]{images/pandora_results/vase/images/02} \end{minipage}& 
		    \begin{minipage}{\figwidth \linewidth}   \includegraphics[width=\linewidth]{images/pandora_results/vase/shapes/colmap}  \end{minipage}& 
		    \begin{minipage}{0.192 \linewidth}   \includegraphics[width=\linewidth]{images/pandora_results/vase/shapes/pandora} \end{minipage}&
		    \begin{minipage}{\figwidth \linewidth}   \includegraphics[width= \linewidth]{images/pandora_results/vase/shapes/ours}  \end{minipage}
		\\
%		\includegraphics[width=\figwidth \linewidth]{images/pandora_results/vase/images/02}&
     \begin{minipage}{\figwidth \linewidth}  \includegraphics[width=\linewidth]{images/pandora_results/vase/azimuth/crop_azimuth_view_2}  \end{minipage}&
	\begin{minipage}{\figwidth \linewidth} 	\includegraphics[width=\linewidth]{images/pandora_results/vase/colmap/photometric_normal_vis/crop_02}  \end{minipage}&
	\begin{minipage}{\figwidth \linewidth} 	\includegraphics[width=\linewidth]{images/pandora_results/vase/pandora/crop_cam_00070000_0}  \end{minipage}&
	\begin{minipage}{\figwidth \linewidth} 	\includegraphics[width=\linewidth]{images/pandora_results/vase/ours/epoch_49/crop_normal_map_view_1}  \end{minipage}
		\vspace{1em}
	\\
	\begin{minipage}{\figwidth \linewidth} \includegraphics[width=\linewidth]{images/pandora_results/owl/images/33}  \end{minipage}&
   \begin{minipage}{0.195 \linewidth}  \includegraphics[width=\linewidth]{images/pandora_results/owl/shapes/colmap}  \end{minipage}& 
  \begin{minipage}{\figwidth \linewidth} 	\includegraphics[width=\linewidth]{images/pandora_results/owl/shapes/pandora}  \end{minipage}&
  \begin{minipage}{\figwidth \linewidth} 	\includegraphics[width=\linewidth]{images/pandora_results/owl/shapes/ours}  \end{minipage}
	\\
	\begin{minipage}{\figwidth \linewidth} \includegraphics[width=\linewidth]{images/pandora_results/owl/azimuth/crop_azimuth_view_33}  \end{minipage}&
	\begin{minipage}{\figwidth \linewidth} \includegraphics[width=\linewidth]{images/pandora_results/owl/colmap/photometric_normal_vis/crop_33}  \end{minipage}&
	\begin{minipage}{\figwidth \linewidth} \includegraphics[width=\linewidth]{images/pandora_results/owl/pandora/crop_cam_00139000_0}  \end{minipage}&
	\begin{minipage}{\figwidth \linewidth} \includegraphics[width=\linewidth]{images/pandora_results/owl/ours/epoch_49/crop_normal_map_view_32}  \end{minipage}
	\\
%		\includegraphics[width=\figwidth \linewidth]{images/pandora_results/vase/azimuth_view_1}&
%%		\includegraphics[width=\figwidth \textwidth]{images/pandora_results/vase/draw_time_2022_11_03_01_30_55/mesh_metashape} &
%		\includegraphics[width=\figwidth \linewidth]{images/pandora_results/vase/draw_time_2022_11_03_01_30_55/pandora_00070000} &
%%		\includegraphics[width=\figwidth\textwidth]{images/pandora_results/vase/draw_time_2022_11_03_01_30_55/mesh_with_half_pi_ambiguity} &
%		\includegraphics[width=\figwidth\linewidth]{images/pandora_results/vase/draw_time_2022_11_03_01_30_55/mesh_ours} 
%		\\
%		\includegraphics[width=\figwidth \linewidth]{images/pandora_results/owl/01.jpg}&
%		\includegraphics[width=\figwidth \linewidth]{images/pandora_results/owl/azimuth_view_1}&
%%		\includegraphics[width=\figwidth \textwidth]{images/pandora_results/owl/draw_time_2022_11_03_02_04_12/mesh_metashape} &
%		\includegraphics[width=\figwidth \linewidth]{images/pandora_results/owl/draw_time_2022_11_03_02_04_12/00130000} &
%%		\includegraphics[width=\figwidth\textwidth]{images/pandora_results/owl/draw_time_2022_11_03_02_04_12/mesh_with_half_pi_ambiguity} &
%		\includegraphics[width=\figwidth\linewidth]{images/pandora_results/owl/draw_time_2022_11_03_02_04_12/mesh_ours} 
%		\\
%		\includegraphics[width=\figwidth \linewidth]{images/pandora_results/gnome/01.jpg}&
%		\includegraphics[width=\figwidth \linewidth]{images/pandora_results/gnome/azimuth_view_1}&
%%		\includegraphics[width=\figwidth \textwidth]{images/pandora_results/gnome/draw_time_2022_11_03_01_49_07/mesh_metashape} &
%		\includegraphics[width=\figwidth \linewidth]{images/pandora_results/gnome/draw_time_2022_11_03_01_49_07/00020000} &
%%		\includegraphics[width=\figwidth\textwidth]{images/pandora_results/gnome/draw_time_2022_11_03_01_49_07/mesh_with_half_pi_ambiguity} &
%		\includegraphics[width=\figwidth\linewidth]{images/pandora_results/gnome/draw_time_2022_11_03_01_49_07/mesh_ours} 
	\end{tabular}
	\caption{Qualitative comparison on PANDORA dataset~\cite{dave2022pandora}. Colmap~\cite{schoenberger2016mvs} breaks down for specular objects. Using only polarimetric azimuth angle maps, MAS shows comparable reconstruction results to the inverse rendering based method~\cite{dave2022pandora} . 
%		Conventional MVS based photoconsistency performs poorly due to severe view dependent specularity.
}
\label{fig.pandora}
\end{figure}
